A halo model for cosmological Lyman-limit systems

We present an analytical model for cosmological Lyman-limit systems (LLSs) that successfully reproduces the observed evolution of the mean free path (L) of ionizing photons. The evolution of the co-moving mean free path is predominantly a consequence of the changing meta galactic photo-ionization rate and the increase with cosmic time of the minimum mass below which halos lose their gas due to photo-heating. In the model, Lyman-limit absorption is caused by highly ionized gas in the outskirt of dark matter halos. We exploit the association with halos to compute statistical properties of LLSs and of their bias, b. The latter increases from 1.5 to 2.6 from redshifts 2 to 6. Combined with the rapid increase with redshift of the bias of the halos that host a quasar, the model predicts a rapid drop in the value of L when measured in quasar spectra from z=5 to 6, whereas the actual value of L falls more smoothly. We derive an expression for the effective optical depth due to Lyman limit absorption as a function of wavelength and show that it depends sensitively on the poorly constrained number density of LLSs as a function of column density. The optical depth drops below unity for all wavelengths below a redshift of 2.5, which is therefore the epoch when the Universe first became transparent to ionizing photons.

==> Attenuation.tex <==
\section{Connecting sinks and sources to the photo-ionization rate}
\label{sect:attenuation}
In this Appendix we examine the relation between the emissivity 
of ionizing photons, the attenuation length, and the amplitude of the ionizing background. We do so by accounting for the frequency dependence of the attenuation. We obtain the same scaling between emissivity and photo-ionization rate, $\epsilon_\nu\propto \Gamma_{-12}^{1/3}$, as found by others 
\cite[e.g][]{Furlanetto05,McQuinn11}, but our expression clarifies how the proportionality constant depends on the \cddf\ and the spectrum of the ionizing sources. We also formulate the result in terms of the clumping factor of the \igm\ - the factor by which recombinations are enhanced over the recombination rate in a uniform \igm.  We start by briefly reviewing how $\epsilon_\nu$, $\Gamma_{-12}$ and \X\ are related by the cosmological radiative transfer equation.

The cosmological radiative transfer equation describes the change in the specific mean intensity, $J_\nu$, along a light ray due to emission and absorption \cite[e.g.][]{Madau99},
\begin{align}
    \left(\frac{\partial}{\partial t}-\nu\,H(z)\frac{\partial}{\partial\nu}+3H\right) J_\nu
    &=-c\,\alpha_\nu\,J_\nu+\frac{c}{4\pi}\epsilon_\nu\,,
\label{eq:cRT}
\end{align}
where $\alpha_\nu$ is the absorption coefficient and $\epsilon_\nu$ the emissivity (in units of energy per unit volume, per unit time, per unit frequency). In this equation, all quantities are  in {\em proper units}, and a subscript $\nu$ indicates frequency dependence.
When applied to hydrogen ionizing photons, which have energy $h\nu\geq h\nu_{\rm th}=1{\rm Ryd}$, this equation can be simplified because such photons travel only a relatively short distance before being absorbed by neutral hydrogen, therefore the redshifting of such photons can be neglected to a first approximation. The formal solution to the resulting equation is given by Eq.~(1.29) in \cite{Rybicki79}, which we write as
\begin{align}
4\pi J_\nu(l)&=\int_0^l\,\epsilon_\nu(l')\,\exp(-\alpha_\nu l')\,dl'\approx \epsilon_\nu\,\int_0^{\alpha_\nu\,l} \frac{\exp(-\tau)}{\alpha_\nu}\,d\tau\,,
\label{eq:Jnu1}
\end{align}
where $J_\nu(l)$ is the angle-averaged specific intensity due to all sources out to a proper distance $l$, $\tau=\int_0^l \alpha_\nu dl$ is the optical depth out to distance $l$; $\epsilon_\nu$ is assumed to be spatially uniform and is taken outside of the integral. The specific intensity due to all sources follows from letting $l\to\infty$.

We can obtain an approximate closed-form expression for $J_\nu(l)$ by neglecting absorption when $\tau<1$, and assuming no radiation reaches the observer from sources for which $\tau>1$. In this \lq local\rq\ or \lq source function\rq\ approximation,
\begin{align}
4\pi J_\nu &\approx \epsilon_\nu\,\lambda_{\rm FP}\,;\quad \lambda_{\rm FP}=\int_0^1\,\frac{d\tau'}{\alpha_\nu(\tau')}\,.
\end{align}
The proper length $\lambda_{\rm FP}$ is the \lq free path\rq\ of the photon (at frequency $\nu$), {\em i.e.} the distance it travels along a given sight line until it encounters an optical depth of $\tau=1$. $\alpha_\nu$ is a constant in space in a homogeneous \igm\ and hence in that case $\lambda_{\rm FP}=1/\alpha_\nu$. However, $\lambda_{\rm FP}$ depends on location and direction in an inhomogeneous \igm, in which case we might be tempted to replace $\lambda_{\rm FP}$ by its spatial average, $\lambda_{\rm MFP}=\langle\lambda_{\rm FP} \rangle$, and relate the average $J_\nu$ to the emissivity via the mean free path, $\lambda_{\rm MF}$
\begin{align}
4\pi \langle J_\nu\rangle &\approx \epsilon_\nu\,\lambda_{\rm MFP}\,,
\label{eq:lmfp}
\end{align}
Since $\lambda_{\rm FP}$ depends on frequency, so does $\lambda_{\rm MFP}$, and we need to average over the spectrum of the sources to relate $\Gamma_{-12}$ to the rate at which ionizing photons are emitted \citep{Madau99}.

Consider now the following alternative derivation. Assume again a homogeneous distribution of sources of ionizing photons with mean emissivity $\epsilon_\nu$. The luminosity emitted by a small volume $dV$ is then $\epsilon_{\nu'}d\nu'\,dV$,
and hence the total luminosity of a spherical shell of radius $l$ and thickness $dl$ is $dL_{\nu'}=\epsilon_{\nu'}\,4\pi\,d_A^2\,dl$, where $d_A$ is the angular diameter distance that corresponds to $l$. The specific mean intensity at $l=0$ due to the sources in this shell is on average
\begin{align}
4\pi\,\langle dJ_\nu\rangle\,d\nu &= \frac{dL_{\nu'}d\nu'}{4\pi d_L^2}\,\exp(-\tau_{\nu, \rm eff}(l))\,dl\,,
\end{align}
where $d_L$ is the luminosity distance that corresponds to $l$. In terms of the values $a_e$ and $a_o$ of the expansion factors at emission and absorption, we have that $d\nu'/d\nu=a_0/a_e$, and $d_A/d_L=(a_e/a_o)^2$. Therefore
\begin{align}
    4\pi\,\langle dJ_\nu\rangle = \left(\frac{a_e}{a_o}\right)^3\,
    \epsilon_{\nu'}\,\exp(-\tau_{\nu, \rm eff}(l))\,dl\,,
\end{align}
where $\tau_{\nu, \rm eff}(l)$ is the effective optical depth at frequency $\nu$ out to distance $l$. Integrating over all shells yields
\begin{align}
4\pi J_\nu &=\int_0^\infty \left(\frac{a_e}{a_o}\right)^3\,\epsilon_{\nu'}\,\exp(-\tau_{\nu, \rm eff}(l))\,dl\,,
\end{align}
where we dropped the $\langle\rangle$ brackets \citep[see, e.g.][]{Madau99}. Using the definition of the attenuation length, $d\tau_{\nu, \rm eff}/dl\equiv 1/\lambda_{\nu, \rm eff}$, from the previous section, allows us to change integration variable from $dl$ to $d\tau_{\nu\,\rm eff}$ and find 
\begin{align}
    4\pi J_\nu &=
    \epsilon_\nu\lambda_{\nu, \rm eff}
    \int_0^\infty \exp(-\tau_{\nu, \rm eff})\,d\tau_{\nu, \rm eff}
    =
    \epsilon_\nu\,\lambda_{\nu, \rm eff}\,,
    \label{eq:JL}
\end{align}
where we assumed that $\epsilon_\nu$ and $\lambda_{\nu, \rm eff}$ are constants in space, and neglected the factor $(a_e/a_o)^3$ which is fine as long as redshifting effects can be neglected over the distance $\lambda_{\nu, \rm eff}$.

We note that the mean free path that appears in 
Eq.~(\ref{eq:lmfp}) depends on optical depth, whereas the attenuation length of Eq.~(\ref{eq:JL}) depends on the {\em effective} optical depth. $\lambda_{\rm MFP}$ and \L\ are sometimes used interchangeably in the literature, even though they are different measures of attenuation. We show this explicitly in Appendix~B, where we compute $\lambda_{\rm MFP}$ and \L\ in a simple toy model in which individual absorbers have the same value of the optical dept, $\tau_i$. We show that $\lambda_{\rm MFP}=\L$ in the case of $\tau_i\to 0$ (a uniform medium) and in the case of $\tau_i\to \infty$. In practice, the optical depth in the \igm\ is dominated by absorbers with $\tau_i\sim 1$ in which case $\L>\lambda_{\rm MFP}$. To us, it makes more sense that $J_\nu$ is related to $\epsilon_\nu$ through the effective optical depth, $\tau_{\rm eff}$, rather than the optical, $\tau$.

We account for the frequency dependence of $\lambda_{\nu, \rm eff}$ as follows. We first approximate the dependence\footnote{We use this approximate frequency dependence in the analytic relations of this paper, yet use the more accurate version of Eq.~(1) of \cite{Verner96} when performing numerical calculations.}
of the photo-ionization cross section on frequency as \citep[e.g.][]{Verner96}
\begin{align}
    \sigma_\nu &=\sigma_{\rm th}\times\left(\frac{\nu}{\nu_{\rm th}}\right)^{-3}\equiv \sigma_{\rm th}\times s(\frac{\nu}{\nu_{\rm th}})\,;
    \label{eq:sigma_nu}
\end{align}
where the function $s(x)\propto x^{-3}$ encodes the frequency dependence of $\sigma_\nu$. The derivation of Eq.~(\ref{eq:X}) shows that $\X\propto \sigma_\nu^{-2/3}\propto \nu^2$: since higher energy photons see a smaller cross section, their attenuation length is longer. This results in the following dependence of the proper attenuation length on frequency,
\begin{align}
    \lambda_{\nu, \rm eff} &= \lambda_{\rm eff}\times\left(\frac{\nu}{\nu_{\rm th}}\right)^2\,,
    \label{eq:l_nu}
\end{align}
and similarly,
\begin{align}
    X_{\nu, \rm eff} &= X_{\rm eff}\times\left(\frac{\nu}{\nu_{\rm th}}\right)^2\,,
    \label{eq:X_nu}
\end{align}
where $\lambda_{\rm eff}$ and \X\ are evaluated at frequency $\nu=\nu_{\rm th}$.
The frequency dependence of Eq.~(\ref{eq:l_nu}) differs from the scaling $\propto \nu^{3/2}$ derived by \cite{Madau99} who assumed that $f(N_{\rm HI})\propto N_{\rm HI}^{-3/2}$, whereas in our model $f(N_{\rm HI})\propto N_{\rm HI}^{-5/3}$. 

We can now integrate Eq.~(\ref{eq:JL}) over frequency by using the frequency dependence of $\lambda_{\nu, {\rm eff}}$ from Eq.~(\ref{eq:l_nu}) to relate the photo-ionization rate, $\Gamma_0$, to the (proper) emissivity of ionizing photons, $\dot n_\gamma$,
\begin{align}
\Gamma_0 &\equiv \Gamma_{-12}\,10^{-12}{\rm s}^{-1}=\int_{\nu_{\rm th}}^\infty \frac{4\pi J_\nu}{h\nu}\,\sigma_\nu\,d\nu
\equiv {\cal N}\,\,\lambda_{\rm eff}\,\sigma_{\rm th}\,\dot n_\gamma
\nonumber\\
\dot n_\gamma &\equiv \int_{\nu_{\rm th}}^\infty
\frac{\epsilon_\nu}{h\nu}\,d\nu\,;\quad 
{\cal N} \equiv {\dot n_\gamma}^{-1}
\int_{\nu_{\rm th}}^\infty 
\frac{\epsilon_\nu}{h\nu}\frac{\nu_{\rm th}}{\nu}\,d\nu\,.
\label{eq:GN}
\end{align}
The dimensionless number ${\cal N}$ depends on the shape of the ionizing spectrum. For a power-law spectrum of the form $\epsilon_\nu\propto \nu^{-\eta}$, ${\cal N}=\eta/(\eta+1)\approx 0.61$, with the numerical value taking $\eta=1.57$ for the average UV spectral slope of quasars from \cite{Haar12UVbackground}. The corresponding value for a black body spectrum of temperature $10^5{\rm K}$ is ${\cal N}=0.54.$

We recall that \L\ that appears in Eq.~(\ref{eq:GN}) itself depends on the value of $\Gamma_{-12}$, see Eq.~(\ref{eq:lambda}). We can eliminate \L\ between these two equations to relate the photo-ionization rate directly to the emissivity of ionizing photons,
\begin{align}
\dot n_\gamma(z) &= 
\frac{1.19\times 10^{52}}{{\cal N}}
\,{\rm s}^{-1}\,{\rm Mpc}^{-3}\,
f_{17.2}(z)\,
\left(\frac{1+z}{4}\right)^3\,
\,\Gamma^{1/3}_{-12}(z)\,.
\label{eq:dotn}
\end{align}
If the ionizing emissivity of photons is known for a given population of sources (e.g. galaxies or quasars), then
Eq.~(\ref{eq:dotn}) predicts the corresponding photo-ionization rate. The strong dependence $\Gamma_{-12}\propto \dot n^3_\gamma$ has been noted before \cite[e.g.][]{McQuinn11}.

Finally, the rate at which ionizing photons are produced equals the rate lost through recombinations, provided the \igm\ is in photo-ionization equilibrium. The recombination rate of the inhomogeneous \igm\ can be defined in terms of that of homogeneous \igm\ by in terms of the clumping factor, ${\cal C}$, 
\begin{align}
\left.\frac{dn_{\rm HI}}{dt}\right|_{\rm rec} &\equiv  {\cal C}\,\alpha_{\rm B}(T)\,n^2_{\rm H}\,.
\end{align}
Combining this with Eq.~(\ref{eq:dotn}) yields a relation between the clumping factor and the amplitude of the \cddf\ and $\Gamma_{-12}$,
\begin{align}
{\cal C}(z)&= \frac{18.3}{{\cal N}}\,
f_{17.2}(z)\,\Gamma^{1/3}_{-12}(z)\,
\left(\frac{1+z}{4}\right)^{-3}\,.
\end{align}
Our value for ${\cal C}(z=3)\approx 18.3/{\cal N}$ is higher than the value of 10 assumed by \cite{Haar12UVbackground}, even though we reproduce their value of \L.

These findings are in line with previous derivations. \cite{Furlanetto05} derive the scalings $\at\propto \Gamma_{-12}^{2/3}$ and $f(N_{\rm HI})\propto \Gamma_{-12}^{-2/3}$, starting from the model of the density probability function ({\sc pdf}) of \cite{MiraldaEscude00}, and \cite{Daloisio18} used similar arguments combined with the Jeans column-density {\em Ansatz} of \cite{Scha01Lya} to find that $\at\propto \Gamma_{-12}^{2/3}$ \cite{McQuinn11} derive the scaling $\Gamma_{-12}\propto \epsilon^{1/(2-\beta)}$, where $\beta$ is the slope of the \cddf, as before. Therefore taking our value of $\beta=5/3$, they also obtain $\Gamma_{-12}\propto\epsilon^3$. Confusingly though, all these models are based on the {\sc pdf} derived by \cite{MiraldaEscude00} which aims to describe the density {\sc pdf} of {\em voids} -  whereas the absorption actually occurs in over dense regions. Therefore it is not clear to what extent these previous models are actually applicable. In contrast, our halo model aims to describe gas in the over dense regions that cause the absorption. It is then gratifying to find that, nevertheless, we obtain the same scaling relations.

==> MFP-calculation.tex <==
\section{Attenuation of ionizing photons}
\label{sect:MFP}
% the sources of ionizing photons, which are thought to be hot stars in galaxies and quasars. However, it additionally depends on the number density of photon sinks. We begin this section by clarifying these two dependencies.
In the previous section we derived an analytical relation for the  evolution of the \cddf\ of highly ionized, strong absorbers, in terms of the mass function of dark matter halos. These absorbers limit the distance that ionizing photons can travel in the post-reionization Universe. That distance is sometimes characterised in terms of a mean free path of ionizing photons, or sometimes in terms of an attenuation length. 
In the literature these are often used interchangeably, however they are in fact not equal to each other.

The {\em mean free path}, hereafter \lam, is defined as follows: consider an ionizing photon travelling a distance $\lambda$ from a source before it encounters cumulatively a total optical depth of $\tau=1$. That distance is the \lq free path\rq\ of that photon, and the mean $\langle \lambda\rangle=\lam$, is the mean free path. The average could be over directions and/or over sources. The {\em attenuation length}, hereafter \at, on the other hand, is defined as follows. The cumulative effect of absorbers decreases the transmission, $F$, in the spectrum of a source as a function of distance. The distance where the transmission falls below $1/e$, on average, is \at. Again the average could be over directions or over sources. Defining the effective optical depth, $\tau_{\rm eff}$, by $\langle F\rangle\equiv \exp(-\tau_{\rm eff})$, means that $\tau_{\rm eff}=1$ at a distance \at\ from the source. We start this section by briefly reviewing how \lam\ and \at\ are related to the \cddf\, and how they are related to each other.

\subsection{Mean free path versus attenuation length}
To simplify the analysis, we assume that all absorbers have the same value of the optical depth, $\tau_i$. Denote the number density of absorbers per unit distance as $\mu$, and assume that the absorbers are uncorrelated and Poisson distributed.

Consider first the case of $\tau_i\to\infty$. In that limit, the free path $\lambda$ is simply the distance from the source to the first absorber. The \pdf\ of $\lambda$ is therefore
\begin{equation}
    {\cal P}(\lambda)=\frac{1}{\mu}{\mathbb P}(0| \mu\lambda)=\frac{1}{\mu}\exp(-\mu\,\lambda)\,,
\end{equation}
where ${\mathbb P}(x|y)=y^x\,\exp(-y)/x!$ is the Poisson distribution. Here, ${\mathbb P}(0| \mu \lambda)$ is the probability that the photon does not encounter any absorber after travelling the distance $\lambda$. The mean of $\lambda$ is \lam, and given by 
\begin{equation}
    \lam=\int_0^\infty\,  \frac{\lambda}{\mu}\,\exp(-\mu\lambda)\,d\lambda=\frac{1}{\mu}\,,
\label{eq:lam1}
\end{equation}
the average distance between absorbers. Consider now the case of $\tau_i\leqslant 1$. The probability of having more than some number $N'$ absorbers in a distance $\lambda$, is given by
\begin{equation}
    {\cal P}(>N'|\lambda)=1-{\cal P}(N=0, 1, 2, \cdots N'|\lambda)
                  =1-\sum_{N=0}^{N'}\,{\mathbb P}(N' | \mu \lambda)\,,
\end{equation}
namely 1 minus the probability of having 0, 1, $\cdots$, $N'$ absorbers in the interval $\lambda$. The probability of reaching $>N'$ absorbers after travelling a distance between $\lambda$ and $\lambda+d\lambda$ is the derivative of this cumulative distribution with respect to $\lambda$, and is the Gamma distribution,
\begin{equation}
    {\cal P}(\lambda)=\frac{\mu\,\exp(-\mu\lambda)\,(\mu \lambda)^{N'-1}}{(N'-1)!}\,.
    \label{eq:pL}
\end{equation}
This is a well-known result in statistics. The \pdf\ of the free path is therefore given by Eq.~(\ref{eq:pL}), provided we set $N'\to 1/\tau_i$. The mean free path is then

\begin{equation}
    \lam=\int_0^\infty d\lambda\,{\cal P}(\lambda)=\frac{(\tau_i^{-1}+1)\,\Gamma(\tau_i^{-1})}{\mu\,(\tau_i^{-1}-1)!} \approx\frac{1}{\tau_i\mu}\,.
    \label{eq:lam2}
\end{equation}

Now we calculate $\at$ for these two cases. Consider first the case of $\tau_i\to\infty$. The mean transmission a distance $\lambda$ from the source is the fraction of paths that did not encounter an absorber,  $\exp(-\tau_{\rm eff}(\lambda))={\mathbb P}(0|\mu \lambda)$. Therefore, the attenuation length is $\lambda_{\rm eff}=\mu^{-1}$, and equals the mean free path, Eq.~(\ref{eq:lam1}): in the case of strong absorbers, \lam\ and \at\ are identical. In the case of $\tau_i\leqslant 1$, the effective optical depth after travelling a distance $\lambda$, is $\tau_{\rm eff}(\lambda)=\mu\,\lambda\,(1-\exp(-\tau_i))$
and the corresponding attenuation length is
\begin{equation}
    \lambda_{\rm eff}=\frac{1}{\mu\,\left(1-\exp(-\tau_i)\right)}\,.
\end{equation}
The attenuation length equals the mean free path, Eq.~(\ref{eq:lam2}), in the limit of $\tau_i\ll 1$, but for $\tau_i=0.5$, for example, $\lam=2/\mu$ but $\at=2.5/\mu$.

In conclusion: in situations where absorption is dominated by either very strong absorbers or very weak absorbers - $\tau_i\to\infty$ or $\tau_i\ll 1$ - the mean free path equals the attenuation length. However, if a significant fraction of the absorption is due to absorbers with optical depth of order unity, then the attenuation length is larger than the mean free path. As we will show below, this is the case for ionizing photons in the \igm, and hence we need to take care to distinguish between these two measures for the distance over which ionizing photons can travel.

From a single observed spectrum, we can only determine \lam, not \at. However, obtaining an accurate measure of \lam\ may be challenging, given that it is hard to measure $\tau_i$ accurately when it is of order unity. Therefore \at\ may be a better measure of the \igm's opacity to ionising photons. In simulations, on the other hand, it may be easier to measure \lam\ than \at. 

Next, we briefly review the relation between the emissivity of ionizing sources, \at, and the photo-ionization rate.

\subsection{Photo-ionization of the \igm}
The {\em cosmological} radiative transfer equation describes the change in the specific mean intensity along a light ray due to emission and absorption \cite[e.g.][]{Madau99},
\begin{equation}
    \left(\frac{\partial}{\partial t}-\nu\,H(z)\frac{\partial}{\partial\nu}+3H\right) J_\nu
    =-c\,\alpha_\nu\,J_\nu+\frac{c}{4\pi}\epsilon_\nu\,,
\label{eq:cRT}
\end{equation}
where $\alpha_\nu$ is the absorption coefficient and $\epsilon_\nu$ the emissivity (in units of energy per unit volume, per unit time, per unit frequency). In this equation, all quantities are  in {\em proper units}, and a subscript $\nu$ indicates frequency dependence.
When applied to hydrogen ionizing photons, which have energy $h\nu\geq h\nu_{\rm th}=1{\rm Ryd}$, this equation can be simplified because such photons travel only a relatively short distance before being absorbed by neutral hydrogen, therefore the redshifting of such photons can be neglected as a first approximation. The formal solution to the resulting equation is given by Eq.~(1.29) in \cite{Rybicki79}, which we write as
\begin{equation}
4\pi J_\nu(l)=\int_0^l\,\epsilon_\nu(l')\,\exp(-\alpha_\nu l')\,dl'\approx \epsilon_\nu\,\int_0^{\alpha_\nu\,l} \frac{\exp(-\tau)}{\alpha_\nu}\,d\tau\,,
\label{eq:Jnu1}
\end{equation}
where $J_\nu(l)$ is the angle-averaged specific intensity due to all sources out to a proper distance $l$, $\tau\equiv\alpha_\nu l$ is the optical depth, and $\epsilon_\nu$ is assumed to be spatially uniform. The specific intensity due to all sources follows from letting $l\to\infty$.

In the \lq local\rq\ or \lq source function\rq\ approximation of \cite{Madau99},
absorption is neglected for $\tau<1$, and assumed to be complete when $\tau>1$.
In this approximation,
\begin{equation}
4\pi J_\nu \approx \frac{\epsilon_\nu}{\langle\alpha_{\nu, {\rm th}}\rangle}\equiv \epsilon_\nu\lambda_{\nu, {\rm th}}\,;\quad
\lambda_{\nu, {\rm th}} \equiv \frac{1}{\langle\alpha_{\nu, {\rm th}}\rangle}\,.
\end{equation}
Here, $\lambda_{\nu, {\rm th}}$ is the attenuation length, we note that it is is evaluated at frequency $\nu=\nu_{\rm th}$. The corresponding photo-ionization rate is then
\begin{equation}
    \Gamma_0 = \int_{\nu_{\rm th}}^\infty \frac{4\pi J_\nu}{h\nu}\,\sigma_\nu\,d\nu
           = \lambda_{\nu, {\rm th}}\,\int_{\nu_{\rm th}}^\infty \frac{\epsilon_\nu}{h\nu}\,\sigma_\nu\,d\nu\,,
           \label{eq:Gamma1}
\end{equation}
where we write the photo-ionization cross section as
\begin{equation}
    \sigma_\nu=\sigma_0\,s(\nu/\nu_{\rm th})\,,
    \label{eq:sigma}
\end{equation}
where $\sigma_0\approx 6.34\times 10^{-18}{\rm cm}^2$ is the value of $\sigma_\nu$ at the threshold (ionization) frequency, and the frequency dependence is approximately $s(x)=x^{-3}$ \citep{Verner96}.


Alternatively, we can account for the frequency dependence of the attenuation length by performing the integral in Eq.~(\ref{eq:Jnu1}) for $l\to\infty$ as 
\begin{equation}
    4\pi J_\nu\approx \frac{\epsilon_\nu}{\langle\alpha_\nu\rangle}\int_0^\infty\,\exp(-\tau)d\tau= \frac{\epsilon_\nu}{\langle\alpha_\nu\rangle}\,,
    \label{eq:Jnu}
\end{equation}
which corresponds to making the approximation that the absorption cross section is spatially constant. In this approximation, the photo-ionization rate is 
\begin{equation}
    \Gamma_0 = \int_{\nu_{\rm th}}^\infty \frac{\epsilon_\nu}{\langle\alpha_\nu\rangle\,h\nu}\,\sigma_\nu\,d\nu
    \,.
    \label{eq:Gamma}
\end{equation}
If absorption is mostly due to low column-density absorbers, then
the frequency dependence of the absorption coefficient will be similar to that of the photo-ionization cross-section, 
$\langle\alpha_\nu\rangle\approx \langle\alpha_{\nu, {\rm th}}\rangle\,(\nu/\nu_{\rm th})^{-3}$, so that
\begin{equation}
    \Gamma_0\approx \lambda_{\nu_{\rm th}}\,\sigma_0\,\int_{\nu_{\rm th}}^\infty\,\frac{\epsilon_\nu}{h\nu}\,d\nu\equiv \lambda_{\nu_{\rm th}}\,\sigma_0\dot n_\gamma\,,
    \label{eq:Gamma2}
\end{equation}
where
\begin{equation}
    \dot n_\gamma=\int_{\nu_{\rm th}}^\infty\,\frac{\epsilon_\nu(z)}{h\nu}\,d\nu\,,
\label{eq:dotn}
\end{equation}
is the rate at which ionizing photons are emitted per unit volume.
Comparing the two expression for $\Gamma_0$ derived here, we note that the contribution of higher frequency photons to the photo-ionization rate is artificially suppressed in Eq.(\ref{eq:Gamma1}) compared to Eq.~(\ref{eq:Gamma2}) - a consequence of using the same value of the attenuation length for all photons, independent of their frequency. Therefore, Eq.~(\ref{eq:Gamma2}) is likely to be a better approximation. From now on, we will use the notation \at\ for $\lambda_{\nu_{\rm th}}$ - the attenuation length at the threshold frequency. We will account for redshifting of photons later on.

\subsection{The attenuation length and the statistics of absorbers}
In the clumpy \igm, absorption of ionizing photons occurs in approximately discrete absorbers with a range of neutral hydrogen column densities. Provided that these absorbers are Poisson distributed ({\em i.e.}, provided we neglect any spatial correlations of absorbers), the effective optical depth per proper distance, $dl$, is \cite[e.g.][]{Meiksin93}
\begin{equation}
    \frac{d\tau_{\rm eff}}{dl} = \int_0^\infty\,\frac{d^2 N}{d l\,d N_{\rm HI}}\,\left(1-\exp(-\tau)\right)\,dN_{\rm HI}\,.
    \label{eq:dtaudl}
\end{equation}
Here, $N$ is the number of absorbers with column density $N_{\rm HI}$ per unit proper distance, and $\tau=\sigma_{\rm th}N_{\rm HI}$ is the optical depth of this absorber. As in the previous section, we transform from proper distance, $dl$, to absorption distance, in order to separate evolution resulting purely from the expansion of the Universe from evolution due to changes in the intrinsic properties of the absorbers. We therefore define the effective optical depth per unit absorption distance, as
\begin{equation}
    \frac{{\rm d}\tau_{\rm eff}}{{\rm d}X} = \int_0^\infty\,f(N_{\rm HI})\,\left(1-\exp(-\tau)\right)\,{\rm d}N_{\rm HI}\,.
    \label{eq:dtaudX}
\end{equation}

Ionizing light travelling an absorption distance $X$ will be attenuated by a factor
$\exp(-\tau_{\rm eff})$. Setting $\tau_{\rm eff}=1$ then defines the {\em attenuation absorption distance}, \X, as
\begin{equation}
    \X(z) = \left(\int_0^\infty\,f(N_{\rm HI},z)\,(1-\exp(-\tau))\,{\rm d}N_{\rm HI}\right)^{-1}\,.
    \label{eq:X}
\end{equation}
We note that any evolution of \X\ is due to evolution of the \cddf, {\em i.e.} due to the fact that the absorbers evolve, rather than simply due to the expansion of the Universe.  


Substituting our expression for the \cddf\ from Eq.~(\ref{eq:fN2}) into the equation for \X\ yields\footnote{The integral over $\tau$ is $1.5\Gamma(1/3)\approx 4.02$, where $\Gamma$ denotes the gamma function - not to be confused with the photo-ionization rate.}
\begin{eqnarray}
    \X(z)&=& 
    \left(
    \frac{f_{17.2}(z)}{\sigma_0\,{\rm cm}^{-2}}\int_0^\infty \tau^{-5/3}\,[1-\exp(-\tau)]\,d\tau]\right)^{-1}\nonumber\\
          &=& \left(4.02\,\frac{f_{17.2}(z)}{\sigma_0\,{\rm cm}^{-2}}
          \right)^{-1}\nonumber\\
        &=& 1.4\times \left(\frac{f_c(z)}{f_c(3)}\,\left(\frac{1+z}{4}\right)^{4/3}\,\left(\frac{\Gamma_0(z)}{10^{-12}{\rm s}^{-1}}\right)^{-2/3}\right)^{-1}\,\nonumber\\
\label{eq:Xmfp}
\end{eqnarray}
{\color{red} TK: something missing in the second line of Eq. \ref{eq:Xmfp}}
{\color{red} TK: define $f_c(z)$ explicitly?}
As discussed in the previous section, the term in brackets evolves approximately $\propto (1+z)^{1.6}\,\Gamma_0(z)^{-2/3}$. Using Eq.~(\ref{eq:dX}) yields
\begin{equation}
    \at(z) = 99\,\left[\frac{f_c(z)}{f_c(3)}\,\left(\frac{1+z}{4}\right)^{13/3}\,\left(\frac{\Gamma_0(z)}{10^{-12}{\rm s}^{-1}}\right)^{-2/3}\right]^{-1}{\rm pMpc}\,.
\label{eq:Lmfp}
\end{equation}
The numerical value is small enough to justify neglecting the redshifting of ionizing photons in Eq.~(\ref{eq:cRT}).


% We follow \cite{Meiksin93} in relating the \cddf\ to the mean-free path of ionizing photons, \lam, for Poisson-distributed absorbers\footnote{We will include the effect of the clustering of absorbers below.}. Their argument goes as follows: an ionizing photon travelling through the highly ionized \igm\ will encounter higher-density regions where the photon has some probability of being absorbed. How far the photon can travel before being absorbed then depends on the number density of absorption lines with a given value of the column density and on how they are distributed. 

% The probability that light with frequency $\nu_{\rm th}$ is absorbed by a single absorber with column-density $N_{\rm HI}$ is $1-\exp(-\tau)$, where $\tau=\sigma_{\rm th}\,N_{\rm HI}$. If there are $N$ absorbers with a range of column densities in a proper distance $l$, and these absorbers are uncorrelated, then the average effective optical depth is
% \begin{equation}
%     \frac{d\tau_{\rm eff}}{dl} = \int_0^\infty\,\frac{d^2 N}{d l\,d N_{\rm HI}}\,\left(1-\exp(-\tau)\right)\,dN_{\rm HI}\,.
%     \label{eq:dtaudl}
% \end{equation}

% The value of $d\tau_{\rm eff}/dl$ evolves because the number density of absorbers changes due to the expansion of the Universe, but also because the intrinsic properties of the absorbers change. Using the absorption distance $dX$ introduced earlier, we can separate the two effects by defining
% the effective optical depth per unit absorption distance,
% \begin{equation}
%     \frac{{\rm d}\tau_{\rm eff}}{{\rm d}X} = \int_0^\infty\,f(N_{\rm HI})\,\left(1-\exp(-\tau)\right)\,{\rm d}N_{\rm HI}\,.
% \end{equation}
% The typical absorption distance that a photon travels before being absorbed is obtained by setting $\tau_{\rm eff}=1$, which yields the \lq mean-free absorption distance\rq\
% \begin{equation}
%     \X(z) = \left(\int_0^\infty\,f(N_{\rm HI},z)\,(1-\exp(-\tau))\,{\rm d}N_{\rm HI}\right)^{-1}\,.
%     \label{eq:X}
% \end{equation}
% We note that any redshift dependence of \X\ is due to evolution of the \cddf, {\em i.e.} due to the fact that the absorbers evolve. We will show below that the part of the \cddf\ that sets \X\ is approximately a power-law,
% \begin{equation}
%     f(N_{\rm HI}, z)\approx f_{17.2}(z)\,\left(\frac{N_{\rm HI}}{10^{17.2}\,{\rm cm}^{-2}}\right)^{-\beta}\,,
%     \label{eq:cddfpower}
% \end{equation}
% with power-law index $\beta\approx 5/3$. Substituting this into Eq.~(\ref{eq:X}) yields
% \begin{equation}
%     \X(z) = \left(\frac{f_{17.2}(z)}{\sigma_{\rm th}}\,\frac{\Gamma(2-\beta)}{\beta-1}\right)^{-1}\,,
% \end{equation}
% where $\Gamma$ is the   {\em gamma function}, not the photo-ionization rate. The corresponding {\em proper} mean-free path is then
% \begin{equation}
%     \lam(z) = \frac{c}{H_0\,(1+z)^3}\,\X(z)\,.
%     \label{eq:lambda}
% \end{equation}
% \lam\ evolves due to the expansion of the Universe, in addition to any evolution of \X.

\subsection{Scalings between \at, $\Gamma_0$, $\epsilon$, and gas clumping}
Equation~(\ref{eq:Gamma2}) appears to imply that the photo-ionization rate is proportional to the emissivity, $\Gamma_0\propto \epsilon$, but this is not correct because the attenuation length, \at, itself depends on $\epsilon$. To clarify the scaling relation between $\Gamma_0$ and $\epsilon$, we use Eq.~(\ref{eq:dotn}) and make the $\Gamma_0$-dependence of \at\ more explicit, by writing Eq.~(\ref{eq:Lmfp}) as
\begin{equation}
    \at(z) = \lambda_{12}(z)\,\left(\frac{\Gamma_0(z)}{10^{-12}{\rm s}^{-1}}\right)^{2/3}\,,
\end{equation}
where $\lambda_{12}(z)$ is the attenuation length at redshift $z$ in case $\Gamma_0=10^{-12}{\rm s}^{-1}$. Combining this with Eq.~(\ref{eq:Gamma2}) yields
\begin{equation}
\frac{\Gamma_0(z)}{10^{-12}{\rm s}^{-1}} = 
\left(\frac{\lambda_{12}(z)\sigma_0\dot n_\gamma(z)}{10^{-12}{\rm s}^{-1}}\right)^3\,,
\end{equation}
which results in scalings of $\Gamma_0\propto \dot n_\gamma^3\propto \epsilon^3$ and $\at\propto\epsilon^2$. Substituting numerical values yields a photon-emissivity of
\begin{equation}
\frac{\dot n_\gamma(z)}{\left({\rm pMpc}\right)^{-3}{\rm s}^{-1}} 
= 1.5\times 10^{52}\,
\frac{f_c(z)}{f_c(3)}\,\left(\frac{1+z}{4}\right)^{13/3}
\left(\frac{\Gamma_0(z)}{10^{-12}{\rm s}^{-1}}\right)^{1/3}\,.
\end{equation}
{\color{red} TK: This equation is not consistent with Eq. \ref{eq:Lmfp}. Should fc(z) in the numerator?}{\color{blue}You are correct, thanks for spotting this}

This derivation assumes that the gas is in photo-ionization equilibrium, $dn_{\rm HI}/dt=0$, therefore the mean recombination rate equals the (mean) photon-emissivity,
$\langle\alpha_r\,n_e\,n_{\rm HII}\rangle=\dot n_\gamma$, where $\langle\rangle$ denotes a volume average. Defining the clumping factor ${\cal C}$ in the usual way, $\langle\alpha_r\,n_e\,n_{\rm HII}\rangle\equiv \langle\alpha_r\rangle{\cal C} \langle n_{\rm H}\rangle^2$, then yields
\begin{equation}
    {\cal C}(z)=20\,\frac{f_c(z)}{f_c(3)}\,\left(\frac{1+z}{4}\right)^{-5/3}
    \left(\frac{\Gamma_0(z)}{10^{-12}{\rm s}^{-1}}\right)^{1/3}\,.
\end{equation}
{\color{red} TK comment: the clumping factor evolves faster than I expect. It should only evolve like: $(1+z)^{0.6}$ if the photo-ionization rate is constant in time and mean free path evolves like $(1+z)^{-5.4}$.}


{\color{red}Compare expression of $\dot n_\gamma$ with the SFRD to compute the mean escape factor}

{\color{red} TK comment: we should be able to calculate the clumping factor from the model without assuming the photo-ionization equilibrium. For example, we can get the PDF and calculate the recombination rate. In this way, we can obtain the clumping factor as a function of photo-ionization rate. Then assuming photo-ionization equilibrium, we could predict the photo-ionization rate from the clumping and mean free path, as well as emissivity. I suspect the result will be self-regulatory: the IGM controls the emissivity.}

\cite{Furlanetto05} derive the scalings $\at\propto \Gamma_0^{2/3}$ and $f(N_{\rm HI})\propto \Gamma_0^{-2/3}$, starting from the model of the density probability function ({\sc pdf}) of \cite{MiraldaEscude00}, and \cite{Daloisio18} used similar arguments combined with the Jeans column-density {\em Ansatz} of \cite{Scha01Lya} to find that $\at\propto \Gamma_0^{2/3}$
\cite{McQuinn11} derive the scaling $\Gamma_0\propto \epsilon^{1/(2-\beta)}$, where $\beta$ is the slope of the \cddf, as before. Therefore taking our value of $\beta=5/3$, they also obtain
$\Gamma_0\propto\epsilon^3$. All these models are based on the the {\sc pdf} derived by
\cite{MiraldaEscude00}.


\begin{figure*}
\includegraphics[width={0.95\textwidth}]{Figures/MF_3panels.png}
\caption{Evolution of the mean-free path in the model by \protect\cite{Theuns21}. {\em Panel (a)}: this model's column-density distribution function obtained by integrating Eq.~(\ref{eq:fN}) at two redshifts $z$ as indicated in the legend. The calculation uses $f_{\rm gas}=0.5$ in Eq.~(\ref{eq:nH}), evaluates the case-A recombination coefficient at a temperature of and $T=2.2\times 10^4{\rm K}$ and the photo-ionization cross-section at 1~{\rm Ryd}, and uses the evolving amplitude of the ionizing background from \protect\cite{Haar12UVbackground}. {\em Panel (b)}: corresponding cumulative mean-free absorption distance (co-moving mean-free path), Eq.~(\ref{eq:X}), at those two redshifts, due to absorbers with column density smaller than $N_{\rm HI}$. The {\em solid curve} includes all halo masses, the {\em dashed} and {\em dotted} curves include halos up to $10^{11}$ and $10^{10}{\rm M}_\odot$ solar masses. {\em Panel (c)}: mean-free path in proper megaparsecs (pMpc) computed from Eq.~(\ref{eq:lambda}) ({\em solid block line}). The {\em shaded area} corresponds to varying $M_{\rm crit}$ (Eq.~\ref{eq:fN}) - the critical halo mass below which halos lose their gas due to photo-evaoporation - by a factor of four around the central value taken from \protect\cite{Okamoto08}; {\em red dots} are the observed values taken from Fig.~8 of \protect\cite{Becker21} (see text for further details).
}
\label{fig:MF1}
\end{figure*}

\begin{figure*}
\includegraphics[width={0.95\textwidth}]{Figures/MF_variations_3panels.png}
\caption{Parameter dependence of the evolution of the mean-free path in the model by \protect\cite{Theuns21}, from left to right: the column-density distribution function (\cddf, panel a), the co-moving mean-free path (panel b) and the proper-mean free-path (panel c). The default choice of parameters is shown in {\em blue} and {\em red} in panel (a) for redshift $z=6$ and 3, and black in panel (c). For a given variation, we keep one or more parameters fixed at their $z=3$ value.  The {\em orange dotted line}) keeps the critical halo-mass $M_{\rm crit}$ constant, the {\em olive dashed line} keeps the photo-ionization rate $\Gamma_0$ constant, and the {\em cyan dot-dashed line} keeps both constant. When both are held constant, the $z=6$ \cddf\ is nearly identical to the $z=3$ \cddf\ and the mean-free absorption distance $X_{\rm MF}$ {\em increases} with $z$ because of the evolution of the number density of halos (and hence of absorbers). Of the two parameters, the evolution of $\Gamma_0$ has a slightly larger impact than that of $M_{\rm crit}$ as can be seen in panel (b) by the fact that $X_{\rm MF}$ evolves less if $\Gamma_0$ is kept constant. {\color{red}TK: need to highlight the observation literature; I think it is Becker and Worseck?}}
\label{fig:MF2}
\end{figure*}

% \subsection{The probability distribution of free paths}
% Any given ionizing photon emanating from a source, will travel some proper distance $\lambda$ before being absorbed. The mean of these distances is the mean free path, $\langle\lambda\rangle=\lam$, as computed in the previous section, where we neglected any clustering of absorbers. In this section we compute the probability distribution of free path lengths, ${\cal P}(\lambda)$, iincluding clustering of absorbers with the sources that emit the ionizing photons. We begin by computing the bias of absorbers.

\subsection{Clustering of absorbers}
\label{sect:bias}
\begin{figure*}
\includegraphics[width={0.95\textwidth}]{Figures/Bias3Panel.png}
\caption{Bias of absorption systems in the halo model, as computed
from Eq.~(\ref{eq:bias1}). {\em Panel (a):} contribution of halos of a given mass to the \cddf at redshift $z=3$. {\em Panel (b):} bias of halos as computed by \col\ \protect\citep{Diemer18COLOSSUS}.
{Panel (c):} Bias for lines of a given column density, $b_{\rm NHI}$ from Eq.~(\ref{eq:bias1}); {\em black circles} show the bias for Lyman-limit systems, $b_{\rm LLs}$ from Eq.~(\ref{eq:biasLLS}) for those same redshifts. The bias of LLs is very close to that of lines with a column density of $10^{17}{\rm cm}^{-2}$. Coloured lines in panels (b) and (c) correspond to different redshifts, as per the legend. See text for discussion.}
\label{fig:Bias}
\end{figure*}


\begin{figure*}
\includegraphics[width={0.95\textwidth}]{Figures/FigMFP.png}
\caption{Statistics of the effective optical depth, $\tau_{\rm eff}$, and of the free path, expressed in terms of the biased absorption distance $Y$ defined in Eq.~(\ref{eq:Y}). {\em Solid lines} are numerical results, obtained by generating Poisson-distributed absorbers numerically; {\em dashed lines} use the analytical approximation described in the text.
{\em Left panel:} Probability distribution of $\tau_{\rm eff}$ for the values $Y$ indicated in the legend. The analytical expression is Eq.~(\ref{eq:taueff}). {\em Central panel:} fraction of paths that reach $\tau_{\rm eff}>1$ within a distance $Y$. The analytical expression is Eq.~(\ref{eq:taugt1}). {\em Right panel:} probability that a path reaches $\tau_{\rm eff}>1$, in a narrow interval $dY$ around $Y$. The analytical expression is Eq.~(\ref{eq:pdfY}). See text for further discussion.
}
\label{fig:MFP}
\end{figure*}


In the previous section we associated strong absorbers with dark matter halos. This allows us to compute the bias of absorbers from the bias of their host halos. Following TT21, the bias of absorbers with a given column-density $N_{\rm HI}$ is

\begin{equation}
b_{N_{\rm HI}}(z) = 
\frac{
\int_{\log M_{\rm crit}(z)}^{\infty}
d\log M_h\,\left(b_{M_h}(z)\times g(N_{\rm HI}, M_h, z)\right)
}
{
\int_{\log M_{\rm crit}(z)}^{\infty}
d\log M_h\,\left(g(N_{\rm HI}, M_h, z)\right)
}\,,
\label{eq:bias1}
\end{equation}
and the bias of {\sc LLs} is
\begin{eqnarray}
&\hphantom{.}&\hspace{-1cm}b_{\rm LLs}(z)=\nonumber\\
&\hphantom{..}&\hspace{-2cm}
\frac{
\int_{17.2}^{\infty} d\log N_{\rm HI}\int_{\log M_{\rm crit}(z)}^\infty d\log M_h\,
{\cal F}_1(M_h, N_{\rm HI}, z)
}
{ 
\int_{17.2}^{\infty} d\log N_{\rm HI}\int_{\log M_{\rm crit}(z)}^\infty d\log M_h\,
{\cal F}_2(M_h, N_{\rm HI}, z)
}\nonumber\\
{\cal F}_1(M_h, N_{\rm HI}, z) &=& b_{M_h}(z)\,N_{\rm HI}\, g(N_{\rm HI}, M_h, z)\nonumber\\
{\cal F}_2(M_h, N_{\rm HI}, z) &=& N_{\rm HI}\, g(N_{\rm HI}, M_h, z)\,.
\label{eq:biasLLS}
\end{eqnarray}
Here, $b_{M_h}(z)$ is the bias of a halo of virial mass $M_h$ at redshift $z$, and column densities are assumed to be expressed in units of cm$^{-2}$. 

The bias computed from Eq.~(\ref{eq:bias1}) for absorbers with a given column density is plotted in panel (c) of Fig.~\ref{fig:Bias}, with colours indicating redshift. Below column densities of $\sim 10^{18.5}{\rm cm}^{-2}$, absorber bias is nearly independent of column density. At first somewhat surprising, we also find that the bias then {\em decreases} with increasing column density, until it reaches a minimum value for $N_{\rm HI}\sim 10^{20}{\rm cm}^{-2}$, after which 
the bias increases again at higher columns.

These trends can be understood by examining panel (a) of
Fig.~\ref{fig:Bias}, where we plot\footnote{We only plot this function at redshift $z=3$, but the trends with halo mass are the same at other redshifts.} the function $g(N_{\rm HI}, z=3)$. Below a column density of $\sim 10^{18.5}{\rm cm}^{-2}$, the contribution of halos as a function of mass varies little with column density, which explains why the bias is nearly independent of $N_{\rm HI}$ as well. At higher columns, the nature of absorbers changes from mostly ionized, at $N_{\rm HI}\leqslant 10^{19}{\rm cm}^{-2}$, to mostly neutral, at $N_{\rm HI}\gtrapprox 10^{20}{\rm cm}^{-2}$. This transition imprints a \rq knee\rq-shaped feature in $g$ and also in the \cddf\ \citep{Zheng02Lya, Theuns21}. Lower mass halos transition at lower values of $N_{\rm HI}$ than higher mass halos. Combined with the fact that lower mass halos have lower bias, this results in a decrease in the bias with increasing $N_{\rm HI}$. Once all halos have transitioned to become mostly neutral, the bias increases rapidly with increasing $N_{\rm HI}$, because in this regime, higher column densities are increasingly associated with more massive halos.

The numerical value of the bias and its evolution with redshift can be understood by also examining panel (b) in Fig.~\ref{fig:Bias}, where we plot the halo bias, $b_{M_h}$, computed using \col\ \citep{Diemer18COLOSSUS}, for various redshifts. Panel (a) shows that a halos in the mass range $10^9-10^{11}M_\odot$ contribute about equally to the \cddf\ at column densities $N_{\rm HI}\leqslant 10^{18.5}{\rm cm}^{-2}$, resulting in a weighted bias of such absorbers of $\sim 1.8$, a bit less than that of halos of mass $10^{11}M_\odot$. With increasing redshift, the contribution of lower mass halos increases compared to that of more massive halos. However, the bias of such lower mass halos increases more rapidly with redshift, so that net result is an increase in bias with $z$.

Finally, panel (c) also shows the bias of LLs computed using Eq.~(\ref{eq:biasLLS}) as filled black dots. With the function $g$ decreasing rapidly with increasing $N_{\rm HI}$, it is not surprising that the bias of LLs is close to that of absorbers with $N_{\rm HI}=10^{17.2}{\rm cm }^{-2}$.

Next, we use the bias of absorbers to calculate the mean free path of photons that themselves emanate from a biased region - with bias factor $b_{\rm source}$ as follows.

\subsection{Clustering and the mean free path}
The average contribution of absorbers to the effective optical depth at a distance $X$ from a source with bias $b_S$,
due to absorbers in a narrow column-density range $dN_{\rm HI}$ and narrow range of absorption distances, follows from Eq.~(\ref{eq:dtaudX}),
\begin{eqnarray}
    \langle d\tau_{\rm eff}\rangle &=& \langle N\rangle\,(1-\exp(-\tau))\nonumber\\
    \langle N\rangle &=& f(N_{\rm HI})\,(1+b_S\,b({\rm NHI})\,\xi(X))\,dN_{\rm HI}\,dX\,,
\end{eqnarray}
where $\tau=\sigma_{\rm HI}N_{\rm HI}$ is the optical depth of a single absorber. The factor $(1+b_S\,b_{\rm NHI}\,\xi(X))$ accounts for linear bias. The correlation function of the mass, $\xi$, is usually expressed in co-moving coordinates, but here we find it more convenient to express distances in units of the absorption distance, $X$. Co-moving distance, $r_c$, is related to absorption distance, $X$, by
\begin{equation}
    dX = \frac{H_0}{c}\,(1+z)^2\,dr_c\,.
\end{equation}
We now take advantage of the our findings that the absorber bias is approximately independent of column density, for column-densities below $10^{19}{\rm cm}^{-2}$ that dominate the contribution to the mean free path. Therefore we replace the absorber bias $b_{N_{\rm HI}}\to b_{\rm LLS}$, the bias at the Lyman-limit, $N_{\rm HI}=10^{17.2}{\rm cm}^{-2}$. We also define the dimensionless variable $dY$ by
\begin{equation}
    dY \equiv dX\,\left(1+b_S\,b_{\rm LLS}\,\xi(X)\right)\,,
    \label{eq:Y}
\end{equation}
with boundary condition $Y=0$ for $X=0$. The statistical properties of the effective optical depth out to absorption distance $X$ depend on $Y$, which we dub \lq biased absorption distance\rq. Using $Y$, rather than $X$, allows us to include the effects of the clustering of absorbers with sources of ionizing photons easily. The average number of absorbers that contribute to $d\tau_{\rm eff}$ is then
\begin{equation}
    \langle N\rangle=f(N_{\rm HI}) dN_{\rm HI}\,dY\,.
\end{equation}

We now assume that these absorbers are Poisson-distributed,
\begin{equation}
    {\cal P}(N) = \mathbb(N| \langle N\rangle) = \mathbb{P}(N|\langle N\rangle) \equiv \frac{\langle N\rangle^{N}\,
    \exp(-\langle N\rangle)}{N!}\,,
\end{equation}
where $\mathbb{P}(n|\mu)$ is the Poisson distribution with mean $\mu$. The \pdf\ of $d\tau_{\rm eff}$ follows by a change of variables,
\begin{equation}
    {\cal P}(d\tau_{\rm eff}) = \mathbb(N| \langle N\rangle)\,\frac{1}{1-\exp(-\tau)}\,,
\end{equation}
with mean $\langle N\rangle\,(1-\exp(-\tau))$ and dispersion 
$\langle N\rangle\,(1-\exp(-\tau))^2$. The effective optical depth $\tau_{\rm eff}$ follows from $d\tau_{\rm eff}$ by integrating over $Y$ and $N_{\rm HI}$.

Although the effective optical depth is simply a linear combination of $d\tau_{\rm eff}$'s, there is no simple relation between the \pdf\ of $N$ and that of $\tau_{\rm eff}$, because a linear sum of Poisson distributed variables is not Poisson distributed (or indeed has any other simple \pdf\footnote{
See \cite{Bohm14}, e.g., for a discussion of such \lq Compound Poisson distributions.}). Of course, we can compute the \pdf\ of $\tau_{\rm eff}$ numerically, by generating Poisson-distributed variables and summing $\tau_{\rm eff}$ in bins of $dN_{\rm HI}$ and $dY$. 

It is possible to obtain an approximate analytical expression for the  \pdf\ of the effective optical depth as follows. At sufficiently low column-density, the mean number of lines that contribute to $\tau_{\rm eff}$, $\langle N\rangle$, may be large enough that the central limit theorem is applicable. In that case, the lines are approximately Gaussian distributed (with mean $\langle N\rangle$ and dispersion $\langle N\rangle$). Integrating over $dN_{\rm HI}$, and integrating over $dY$ out to a biased absorption distance $Y$, then corresponds to summing over independently-distributed Gaussian variables. Therefore, the sum is also Gaussian distributed, with a mean the sum of the means, and dispersion the sum of the dispersions. We will denote the value of $\tau_{\rm eff}$ due to these low column-density lines by $\tau_{\rm eff, low}$, and its \pdf\ is
\begin{eqnarray}
    {\cal P}_G(\tau_{\rm eff, low}|\mu, \sigma) &=& \frac{1}{(2\pi\sigma^2)^{1/2}}\,\exp(-\frac{(\tau_{\rm eff, low}-\mu)^2}{2\sigma^2})\nonumber\\
    \mu(Y) &=& Y\,\int_0^{\rm N_{\rm HI, low}}\,f(N_{\rm HI})\,(1-\exp(-\tau))\,dN_{\rm HI}\nonumber\\
    \sigma^2(Y) &=& Y\,\int_0^{\rm N_{\rm HI, low}}\,f(N_{\rm HI})\,(1-\exp(-\tau))^2\,dN_{\rm HI}\,.\nonumber\\
\end{eqnarray}

We now take $N_{\rm HI, low}=10^{17.2}\,{\rm cm}^{-2}$. In that case, the weighting factor $(1-\exp(-\tau))\approx 1$ for those lines with $N_{\rm HI}\ge N_{\rm HI, low}$. The \pdf\ due to these higher column-density lines is now a sum of independently distributed Poisson variables, hence also a Poisson distributed variable. Denoting the value of $\tau_{\rm eff}$ due to these high column-density lines by $\tau_{\rm eff, high}$, we find that its \pdf\ is given by
\begin{eqnarray}
    {\cal P}(\tau_{\rm eff, high}) &=& \mathbb{P}(N|N_P)\nonumber\\
    N_P(Y) &=& Y\,\int_{N_{\rm N_{\rm HI, low}}}^\infty\,dN_{\rm HI}\,.
\end{eqnarray}

The total effective optical depth is $\tau_{\rm eff, low}+\tau_{\rm eff, high}$, with \pdf\
\begin{equation}
    {\cal P}(\tau_{\rm eff}(Y))=\sum_{N=0}^\infty\,
    \mathbb{P}(N|N_P)\,{\cal P}_G(\tau_{\rm eff}-N|\mu, \sigma)\,,
    \label{eq:taueff}
\end{equation}
where $\mu$, $\sigma$ and $N_P$ all proportional to $Y$. The mean of this distribution is the sum of the means of 
$\tau_{\rm eff, low}$ and $\tau_{\rm eff, high}$, 
\begin{eqnarray}
    \langle\tau_{\rm eff}(Y)\rangle &=&Y\,
    \int_0^\infty f(N_{\rm HI})\,\left(1-\exp(-\tau)\right)\,dN_{\rm HI}\nonumber\\
    &\approx& \frac{3}{2}Y\,\frac{f_{17.2}}{\sigma_{\rm HI}}\,,
\end{eqnarray}
where we used the power-law approximation to the \cddf\ of Eq.~(\ref{eq:fN2}).

We can use this to compute the fraction of paths that reach $\tau_{\rm eff}>1$ for a given value $Y$ of the biased absorption distance,
\begin{eqnarray}
    {\cal P}(\tau_{\rm eff}>1|Y)&=&\int_1^\infty {\cal P}(\tau_{\rm eff}|Y)\,d\tau_{\rm eff}\nonumber\\
    &=&\frac{1}{2}\sum_{N=0}^\infty \mathbb{P}(N|N_P)\left\{1\pm {\rm Erf}(x)\right\}\nonumber\\
    x&\equiv&\frac{1-N-\mu}{(2\sigma^2)^{1/2}}\,.
    \label{eq:taugt1}
\end{eqnarray}
Here, ${\rm Erf}$ denotes the error function, and the upper and lower signs applies to the case where $x$ is negative or positive. The fraction of paths that reach $\tau_{\rm eff}$ between $Y$ and $Y+dY$ follows by taking the derivative with respect to $Y$,
\begin{eqnarray}
    {\cal P}(\tau_{\rm eff}=1,Y)
    &=&\frac{d{\cal P}(\tau_{\rm eff}>1|Y)}{dY}\nonumber\\
    &=&\sum_{N=0}^\infty\left\{ \left(\frac{N}{N_P}-1\right)\,\mathbb{P}(N|N_P)\,\left\{1\pm {\rm Erf}(\mp x)\right\}\,\frac{N_P}{Y}\right.\nonumber\\
    &+&\left. \mathbb{P}(N|N_P)\,\frac{\exp(-x^2)}{\pi^{1/2}}\left(\frac{x}{2Y}+\frac{\mu_G}{(2\sigma^2)^{1/2}Y}\right)\right\}\,.
    \label{eq:pdfY}
\end{eqnarray}

These results are illustrated in Fig.~\ref{fig:MFP}. We have generated Poisson-distributed absorption lines, drawn from the \cddf\ of Eq.~(\ref{eq:fN2}) setting $f_{17.2}=1.1\times 10^{-18}$, in narrow bins of $dN_{\rm HI}$ and $dY$, for which \X=1.4. Summing over these allows us to compute $\tau_{\rm eff}$ for a given value of the biased absorption distance $Y$, the fraction of paths that reach $\tau_{\rm eff}>1$ within a given value of $Y$, and the fraction of paths that reach $\tau_{\rm eff}>1$ in a narrow interval $dY$ around $Y$. These are shown as solid lines in panels (a)$\to$(c). The corresponding analytical expressions, Eqs.~(\ref{eq:taueff}), (\ref{eq:taugt1}) and (\ref{eq:pdfY}) are plotted with dashed lines. When $Y$ is small - case Y=1.2 in panel (a) -  the \pdf\ of $\tau_{\rm eff}$ has two clear maxima, which correspond to 0 or 1 strong absorbers contributing to $\tau_{\rm eff}$ (there are further oscillations visible, due to 2 or more strong absorbers). Absorbers with $\tau\lessapprox 10^{17.2}{\rm cm}^{-2}$, which in the analytical model contribute to $\tau_{\rm eff, low}$, are sufficiently rare that approximating their \pdf\ as Gaussian is not a very accurate. This is the reason that the analytical model differs substantially from the numerical calculation for small values of $Y$. As $Y$ increases, such absorbers become more common, and the approximation improves. The analytical model reproduces rather well the fraction of paths that reach $\tau_{\rm eff}>1$ within a given distance $Y$, as shown in panel (b). The derivative of this function with respect to $Y$ is the probability that a given path reaches $\tau_{\rm eff}>1$ in a small interval $dY$ around $Y$, and is plotted in panel (c). The peak of the analytical approximation is a bit narrower than that of the numerical result, but the location of the maximum is very close. Both functions have a long tail to large values of $Y$, with the analytical approximation reproducing the numerical result well.





Bias of first QSOs: see e.g. \cite{Latif22} - halo mass is $1.2\times 10^{12}M_\odot$ at $z=6$.

{\color{red} Need figure that relates $X$ to $Y$}








 

% which is a Poisson distribution with mean $\bar N_A\,(1-\exp(-\tau))$. The total effective optical depth out to absorption distance $X$, $\tau_{\rm eff}$, follows by integrating $d\tau_{\rm eff}$ over column density and distance. We now take account of the fact that the sum of independently distributed Poisson variables is again Poisson distributed, with a mean equal to the sum of the means of these independent variables. Therefore the effective optical depth
% out to a given absorption distance $X$ from a source with bias parameter $b_S$,
% is Poisson distributed
% \begin{equation}
%     {\cal P}_X(\tau_{\rm eff}) = \mathbb{P}\left(\tau_{\rm eff} | \bar\tau_{\rm eff}(X)\right)\,,
% \label{eq:Poisson}
% \end{equation}
% with mean
% \begin{eqnarray}
%     \bar\tau_{\rm eff}(X) &=& \int_0^X\,dX\,\int_0^\infty dN_{\rm HI}\,
%     f(N_{\rm HI})\nonumber\\
%     &\times & \,\left\{1+b_S\,b(N_{\rm HI})\,\xi(X)\right\}\,\left(1-\exp(-\tau)\right)\nonumber\\
%     &\approx& \left.\frac{d\tau_{\rm eff}}{dX}\right|_{\rm b=0}\int_0^X\,dX\ 
%     \left\{1+b_S\,b_{\rm LLS})\,\xi(X)\right\}\,.
% \label{eq:tauX}
% \end{eqnarray}
% The approximation in the last line takes advantage of the fact that the bias of absorbers, $b(N_{\rm HI})$, depends little on column density, so we can replace it approximately by the bias of LLSs, $b_{\rm LLS}\equiv b(N_{\rm HI}=10^{17.2}{\rm cm}^{-2})$.
% The double integral over $N_{\rm HI}$ and $X$ then becomes a single integral over $X$. The factor $\left.(d\tau_{\rm eff}/dX)\right|_{\rm b=0}$ is the effective optical depth per unit absorption distance in case the bias is zero, from Eq.~(\ref{eq:dtaudl}).

% To find the probability distribution for travelling a given distance, it is convenient to define $t$, which is the effective optical depth in units of its mean, $t\equiv \tau_{\rm eff}/\bar\tau_{\rm eff}$. This variable is Poisson distribute with $\bar t=1$. In terms of $t$, the probability that $\tau_{\rm eff}>1$, after travelling an absorption distance $X$, is
% \begin{equation}
%     {\cal P}(\tau_{\rm eff}>1, X) = \int_{1/\bar\tau_{\rm eff}(X)}^\infty\,\mathbb{P}(t|1)\,dt\,.
% \end{equation}
% The fraction of paths that reach $\tau_{\rm eff}=1$ between $X$ and $X+dX$ is therefore
% \begin{eqnarray}
%     {\cal P}(\tau_{\rm eff}=1, X) &=& \frac{d{\cal P}(\tau_{\rm eff}>1)}{dX}\nonumber\\
%     &=& \frac{1}{\bar\tau_{\rm eff}^2}\,
%     \mathbb{P}(1|\bar\tau_{\rm eff})\,\,\frac{d\bar\tau_{\rm eff}}{dX}\nonumber\\
%     &=& \frac{\bar\tau_{\rm eff}^{-1}\,\exp(-\bar\tau_{\rm eff})}{\Gamma(2)}\,
%     \frac{d\bar\tau_{\rm eff}}{dX}\,,
% \label{eq:Ptau}
% \end{eqnarray}
% where $\bar\tau_{\rm eff}(X)$ is given by Eq.~(\ref{eq:tauX}), so that the derivative is
% \begin{equation}
% \frac{d\bar\tau_{\rm eff}}{dX} = \left.\frac{d\tau_{\rm eff}}{dX}\right|_{\rm b=0}\,
%     \left\{1+b_S\,b_{\rm LLS})\,\xi(X)\right\}\,.
% \end{equation}
% Integrating Eq.~(\ref{eq:Ptau}) over alll paths yields
% \begin{equation}
%     \int_0^\infty {\cal P}(\tau_{\rm eff}=1, X)\,dX
%     =\frac{1}{\Gamma(2)}\int_0^\infty x^{-1}\,\exp(-x)\,dx=1\,,
% \end{equation}
% showing that ${\cal P}(\tau_{\rm eff}=1, X)$ is correctly normalized. 





% \begin{equation}
% {\cal P}(\tau_{\rm eff}>1, X) = \int_1^\infty {\cal P}_X(\tau_{\rm eff})\,d\tau_{\rm eff}\,.
% \end{equation}
% The fraction of paths that reach $\tau_{\rm eff}=1$ between $X$ and $X+dX$ is therefore
% \begin{equation}
%     {\cal P}(\tau_{\rm eff}=1, X) = \frac{d{\cal P}_X(\tau_{\rm eff}>1)}{dX}\,.
% \end{equation}













% \subsection{Free path distribution with Poisson Approximation}



% In this section, we calculate the distribution of free paths from the column density distribution. We assume the intergalactic medium contains discrete absorbers with column density $N_{\rm HI}$, distributed according to the column density distribution. We further assume the absorber distribution (with $N_{\rm HI}$), $P(N_{\rm abs}(HI), N_{\rm HI}, X)$, is Poissonian. We assume the number of absorbers is large (>10), so we can approximate the distribution as Gaussian, i.e. the probability of finding the number of absorbers between $N_{\rm abs}$ and $N_{\rm abs}'$ is
% \begin{align}
% &\int^{N_{\rm abs}'}_{N_{\rm abs}} {\rm d}N_{\rm abs} P(N_{\rm abs}, N_{\rm HI}, X)\nonumber\\
% =& \int^{N_{\rm abs}'}_{N_{\rm abs}} {\rm d}N_{\rm abs} P_{\rm Gaussian}(N_{\rm abs}, \mu=\bar{N}_{\rm abs},\sigma^2=\bar{N}_{\rm abs}),
% \end{align}
% where $\bar{N}_{\rm abs}$ is the mean number of $N_{\rm HI}$ absorbers, obtained from the column density distribution:
% \begin{align}
% \bar{N}_{\rm abs} = \int\mathrm{d} N_{\rm HI}\mathrm{d} X\frac{\mathrm{d} N}{\mathrm{d} N_{\rm HI}\mathrm{d} X}
% \end{align}

% The (effective) optical depth $\tau$ given a path length $X$ and $N_{\rm HI}$ due to $N_{\rm abs}$ absorbers is
% \begin{align}
% \tau(X,N_{\rm HI}) = N_{\rm abs} [1-\exp(-N_{\rm HI}\sigma)].
% \end{align}
% We then change the variable from $N_{\rm abs}$ to $\tau$:
% \begin{align}
% &P(N_{\rm abs}, N_{\rm HI}, X){\rm d}N_{\rm abs}\nonumber\\
% =&\frac{P(\tau/[1-\exp(-N_{\rm HI}\sigma)], N_{\rm HI}, X)}{1-\exp(-N_{\rm HI}\sigma)}{\rm d}\tau,
% \end{align}
% which is a Gaussian:
% \begin{align}
% P_{\rm Gaussian}(\tau) = \frac{P(\tau/[1-\exp(-N_{\rm HI}\sigma)], N_{\rm HI}, X)}{1-\exp(-N_{\rm HI}\sigma)},
% \end{align}
% with a scaled mean and variance:
% \begin{align}
% \mu &= \bar{N}_{\rm abs} [1-\exp(-N_{\rm HI}\sigma)],\nonumber\\ \sigma^2 &= \bar{N}_{\rm abs} [1-\exp(-N_{\rm HI}\sigma)]^2.
% \end{align}


% Since the sum of Gaussians are also Gaussian (if the absorbers with different $N_{\rm HI}$ is independently distributed), the probability distribution of $\tau$ summed over all $N_{\rm HI}$ and $X$ is a Gaussian $P(\tau,\mu(X),\sigma^2(X))$ with
% \begin{align}
% \mu(X) &= \int\mathrm{d} N_{\rm HI}\mathrm{d} X\frac{\mathrm{d} N}{\mathrm{d} N_{\rm HI}\mathrm{d} X}[1-\exp(-N_{\rm HI}\sigma)],\nonumber\\ 
% \sigma^2(X) &= \int\mathrm{d} N_{\rm HI}\mathrm{d} X\frac{\mathrm{d} N}{\mathrm{d} N_{\rm HI}\mathrm{d} X}[1-\exp(-N_{\rm HI}\sigma)]^2,
% \end{align}
% integrated over a path length $X$.


% The probability that $\tau>1$ is then
% \begin{align}
% P(\tau>1,X)=\int_1^\infty {\rm d} \tau P(\tau,X).
% \end{align}
% We can then derive the probability of reaching $\tau=1$ within $X$ and $X+{\rm d}X$:
% \begin{align}
% P(\tau=1,X) = \frac{{\rm d}P(\tau>1,X)}{{\rm d} X}.
% \end{align}
% This corresponds to the free path distribution in the unit of path length, if we define the free path as the length where the optical depth reaches unity ($\tau=1$).





